Technical Report for "User-Centric Participatory Sensing: A Game Theoretic Analysis"

Participatory sensing (PS) is a novel and promising sensing network paradigm for achieving a flexible and scalable sensing coverage with a low deploying cost, by encouraging mobile users to participate and contribute their smartphones as sensors. In this work, we consider a general PS system model with location-dependent and time-sensitive tasks, which generalizes the existing models in the literature. We focus on the task scheduling in the user-centric PS system, where each participating user will make his individual task scheduling decision (including both the task selection and the task execution order) distributively. Specifically, we formulate the interaction of users as a strategic game called Task Scheduling Game (TSG) and perform a comprehensive game-theoretic analysis. First, we prove that the proposed TSG game is a potential game, which guarantees the existence of Nash equilibrium (NE). Then, we analyze the efficiency loss and the fairness index at the NE. Our analysis shows the efficiency at NE may increase or decrease with the number of users, depending on the level of competition. This implies that it is not always better to employ more users in the user-centric PS system, which is important for the system designer to determine the optimal number of users to be employed in a practical system.

==> app-proof-mcs0.tex <==
\begin{proof}
On one hand, if one of the conditions in \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3} is not satisfied, then the strategy $\bs_i $ is not feasible as explained early. Thus,  if $\bs_i $ is feasible,   the conditions \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3} must be satisfied.
One the other hand, if  \eqref{eq:mcs-fs1}-\eqref{eq:mcs-fs3} are satisfied, the strategy $\bs_i $ can be implemented by user $i$ successfully, hence is feasible.
\end{proof}


==> app-proof-mcs1.tex <==

%\subsection{Proof for Lemma \ref{lemma:mcs:potential}}\label{app:5}


\begin{proof}
To prove that the Task Selection Game $\T$ is a potential game with the potential function  $\Phi(\bs)$ given in \eqref{eq:xxx:pf}, we   need to show that for every user $i\in \N$ and any  strategies $\bs_i,\bs_i' \subseteq \S_i $ of user $i$, the following equation holds:
\begin{equation}\label{eq:pf-proof}
 \u_i (\bs_i, \bs_{-i} ) - \u_i (\bs_i', \bs_{-i} )
=
\Phi (\bs_i, \bs_{-i} ) - \Phi (\bs_i', \bs_{-i} ),
\end{equation}
under any feasible strategy profile $\bs_{-i}$ of other users.

We first show that   \eqref{eq:pf-proof} holds when user  $i$ only changes the execution order,
while not changing the task selection. Namely, $\bs_i $ and $\bs_i' $ contain the same task set (but different execution orders).
It is easy to see that
\begin{equation}
M_k (\bs_i, \bs_{-i}) = M_k (\bs_i', \bs_{-i}), \quad \forall k\in\S,
\end{equation}
that is, the number of users executing each task $k \in \S$ does not change  when user $i$ only changes the execution order. This implies that the achieved reward and the incurred execution cost of user $i$ will not change.
Thus, by \eqref{eq:xxx:payoff}, we have:
\begin{equation}
\begin{aligned}
& \u_i (\bs_i, \bs_{-i} ) - \u_i (\bs_i', \bs_{-i} ) =
c_i^{\textsc{tr}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i'),
\end{aligned}
\end{equation}
where only the travelling cost of user $i$ is changed.
For the potential function  in \eqref{eq:xxx:pf}, we also have:
\begin{equation}
\begin{aligned}
\Phi (\bs_i, \bs_{-i} ) - \Phi (\bs_i', \bs_{-i} ) =
c_i^{\textsc{tr}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i').
\end{aligned}
\end{equation}
This is because the change of user $i$'s execution order does not affect the execution costs and travelling costs of other users. Based on the above, we can see that   \eqref{eq:pf-proof} holds when user $i$ changes the execution order only.


We then show that   \eqref{eq:pf-proof} holds when player $i$ changes his strategy from $\bs_i $ to $\bs_i' $ by removing a task $\tau \in \bs_i$, i.e., $\bs_i' = \bs_i / \{ \tau \}$.
According to \eqref{eq:xxx:payoff}, we have:
\begin{equation*}
\begin{aligned}
& \u_i (\bs_i, \bs_{-i} ) - \u_i (\bs_i', \bs_{-i} )
%\\
%= &  \sum_{k \in \bs_i }  \frac{V_k}{M_k (\bs_i , \bs_{-i})}
% -
%c_i^{\textsc{ex}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i)
%\\
%&
%-
%\sum_{k \in \bs_i'}  \frac{V_k}{M_k (\bs_i', \bs_{-i})}
%+
%c_i^{\textsc{ex}} (\bs_i') + c_i^{\textsc{tr}} (\bs_i')
\\
= & \ \frac{V_\tau}{M_\tau (\bs_i , \bs_{-i})}  +
c_i^{\textsc{ex}} (\bs_i') + c_i^{\textsc{tr}} (\bs_i') -
c_i^{\textsc{ex}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i) .
\end{aligned}
\end{equation*}
For the potential function  in \eqref{eq:xxx:pf}, we   also have: 
%\begin{figure*}[ht]
% \begin{multicols}{2} 
\begin{equation*}\label{eq:proofxxxx}
\begin{aligned}
& \Phi (\bs_i, \bs_{-i} ) - \Phi (\bs_i', \bs_{-i} )
%\\
%= &  \sum_{k \in \S}   \sum_{m=1}^{M_k(\bs_i, \bs_{-i})} \frac{V_k}{m}
% - \sum_{j\in\N} c_j^{\textsc{ex}} (\bs_j)
% - \sum_{j\in\N} c_j^{\textsc{tr}} (\bs_j)
% \\
%&
%\hspace{-10mm} - \sum_{k \in \S} \!\!\!\!  \sum_{m=1}^{M_k(\bs_i', \bs_{-i})} \frac{V_k}{m}
%+ \sum_{j\neq i} c_j^{\textsc{ex}} (\bs_j)
% + \sum_{j\neq i} c_j^{\textsc{tr}} (\bs_j)
% + c_i^{\textsc{ex}} (\bs_i')+ c_i^{\textsc{tr}} (\bs_i')
% \\
% = &  \!\!\!\!  \sum_{m=1}^{M_\tau(\bs_i, \bs_{-i})}  \frac{V_\tau}{m}  -  \!\!\!\!  \sum_{m=1}^{M_\tau(\bs_i', \bs_{-i})} \frac{w_\tau}{m}
%  +
%c_i^{\textsc{ex}} (\bs_i') + c_i^{\textsc{tr}} (\bs_i') -
%c_i^{\textsc{ex}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i)
 \\
 = & \ \frac{V_\tau}{M_\tau (\bs_i , \bs_{-i})}  +
c_i^{\textsc{ex}} (\bs_i') + c_i^{\textsc{tr}} (\bs_i') -
c_i^{\textsc{ex}} (\bs_i) - c_i^{\textsc{tr}} (\bs_i), 
\end{aligned}
\end{equation*}
%\end{multicols}
%\end{figure*}
which follows because  $ M_\tau(\bs_i , \bs_{-i}) = M_\tau(\bs_i', \bs_{-i}) + 1$ and $ M_k(\bs_i , \bs_{-i}) = M_k(\bs_i', \bs_{-i}) $ for all $k \neq \tau$.
Based on the above, we can see that   \eqref{eq:pf-proof} holds when user $i$ removes a task from his strategy.
Similarly, we can show that    \eqref{eq:pf-proof} holds when user $i$ adds a task into his strategy.

Using the above results iteratively, we can show that
the  equation \eqref{eq:pf-proof} holds when user $i$ changes his strategy from an arbitrary $\bs_i $ to an arbitrary $\bs_i' $.
\end{proof}


==> app-proof-mcs2.tex <==
%\subsection{Proof for Lemma \ref{lemma:mcs:NE}}\label{app:6}

\begin{proof}
We will show that the outcome $\bs^*$ given by \eqref{eq:xxx:NE} is an NE of  $\T$.
According to \eqref{eq:xxx:NE}, we find that for any $i \in \N$,
$$
\Phi(\bs_i^*, \bs_{-i}^*) \geq \Phi(\bs_i ', \bs_{-i}^*), \quad \forall \bs_i ' \subseteq \S_i.
$$
By Lemma \ref{lemma:mcs:potential}, we further have: for any   $i\in \N$ and $\bs_i ' \subseteq \S_i$,
$$
 \u_i (\bs_i^*, \bs_{-i}^* ) - \u_i (\bs_i', \bs_{-i}^* )
=
\Phi (\bs_i^*, \bs_{-i}^* ) - \Phi (\bs_i', \bs_{-i}^* ).
$$
Hence, we have the following observations:
$$
 \u_i (\bs_i^*, \bs_{-i}^* ) \geq \u_i (\bs_i', \bs_{-i}^* ), \quad \forall \bs_i ' \subseteq \S_i, i\in\N,
$$
which implies that the outcome $\bs^*$ in \eqref{eq:xxx:NE} is an NE of  $\T$.
\end{proof}

==> app-proof-mcs3.tex <==

%\subsection{Proof for Lemma \ref{lemma:mcs:tax}}\label{app:7}


\begin{proof}
This lemma can be proved by Theorem \ref{thm:efficiency} and Lemma \ref{lemma:fair1} directly.
\end{proof}

==> section6-reference-bk.tex <==
%!TEX root = Tax_Game_main.tex
%SourceDoc Tax_Game_main.tex

\begin{thebibliography}{1}


%\bibitem{game-theory}
%T.~Basar and G.~Olsder, \emph{Dynamic Noncooperative Game Theory},
%Academic Press, London, 1982.

%\bibitem{game-theory1991}
%R.B.~Myerson, \emph{Game Theory: Analysis of Conflict}, Harvard University, 1991.

\bibitem{game-theory1994}
M.J.~Osborne and A. Rubinstein, ``A Course in Game Theory,'' \emph{MIT Press}, 1994.

%\bibitem{game-theory2005}
%M.J.~Osborne,  \emph{An Introduction to Game Theory}, Oxford University Press, Oxford, 2005.

\bibitem{game-Nash}
J.F.~Nash, ``Equilibrium Points in n-Person Games,''
\emph{Proc.~Nat.~Acad.~Sci.}, pp.48-49, 1950.

\bibitem{app-spectrum1}
X.~Kang, R.~Zhang, and M.~Motani, ``Price-based resource allocation for spectrum-sharing femtocell networks: A stackelberg game approach,''
\emph{IEEE Journal on Selected areas in Communications}, pp.538-549, 2012.

%\bibitem{app-power1}
%C.U.~Saraydar, N.B.~Mandayam, and D.J.~Goodman, ``Efficient Power Control via Pricing in Wireless Data Networks,''
%\emph{IEEE transactions on Communications}, 50(2), 291-303, 2002.

\bibitem{app-power2}
U.O.~Candogan, I.~Menache, A.~Ozdaglar, and P.A.~Parrilo, ``Near-Optimal Power Control in Wireless Networks: A Potential Game Approach,''
\emph{Proc.~IEEE INFOCOM}, pp.1-9, 2010.

\bibitem{app-access1} %% tpc
K.~Khalil and E.~Ekici, ``Multiple Access Game with a Cognitive Jammer,''
\emph{Proc.~IEEE ASILOMAR}, pp.1383-1387, 2012.


\bibitem{app-resource1} %% tpc
H.~Xu and B.~Li, ``Efficient Resource Allocation with Flexible Channel Cooperation in OFDMA Cognitive Radio Networks,''
\emph{Proc.~IEEE INFOCOM}, pp.1-9, 2010.

\bibitem{app-resource2}
J.~Huang, Y.~Yin, Y.~Zhao, Q.~Duan, W.~Wang, and S.~Yu,  %% tpc
``A Game-Theoretic Resource Allocation Approach for Intercell Device-to-Device Communications in Cellular Networks,''
\emph{IEEE Transactions on Emerging Topics in Computing}, pp.1-11, 2014.


\bibitem{app-routing1}
Q.~Zhu, Z.~Yuan, J.B.~Song, Z.~Han, and T.~Basar,
``Interference Aware Routing Game for Cognitive Radio Multi-Hop Networks,''
\emph{IEEE Journal on Selected Areas in Communications}, 30(10), 2006-2015, 2012.

\bibitem{app-relay1}
W.~Zhong, G.~Chen, S.~Jin, and K.K.~Wong,
``Relay Selection and Discrete Power Control for Cognitive Relay Networks via Potential Game,''
\emph{IEEE Transactions on Signal Processing}, 2014.

\bibitem{game-book2012}
Z.~Han, \emph{Game Theory in Wireless and Communication Networks: Theory, Models, and Applications},  Cambridge University Press, 2012.

%\bibitem{game-survey2006}
%E.~Altman, \emph{et al.},
%``A Survey on Networking Games in Telecommunications,''
%\emph{Computer Operation Research}, pp.286-311, 2006.
%
%\bibitem{game-survey2012}
%H.~Shi, W.~Wang, N.~Kwok, and S.~Chen,
%``Game Theory for Wireless Sensor Networks: A Survey,''
%\emph{Sensors}, 12(7), 9055-9097, 2012.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\bibitem{Pareto-1991}
%D.~Fudenberg and J.~Tirole, ``Nash Equilibrium: Multiple Nash Equilibria, Focal Points, and Pareto Optimality,''
%\emph{Game Theory}, pp.18-23, 1991.

\bibitem{Pareto-2008}
P.M.~Pardalos, A.~Migdalas, and L.~Pitsoulis (Ed), \emph{Pareto Optimality, Game Theory and Equilibria}, Springer Science \& Business Media, 2008.

\bibitem{PoA-1999}
E.~Koutsoupias and C.~Papadimitriou,
``Worst-Case Equilibria,''
\emph{Annual Symposium on Theoretical Aspects of Computer Science}, Springer, pp.404-413, 1999.

\bibitem{PoA-2008}
H.~Youn, M.T.~Gastner, and H.~Jeong, ``Price of Anarchy in Transportation Networks: Efficiency and Optimality Control,''
\emph{Physical Review Letters}, 101(12), 2008.

\bibitem{PoAS-2005}
G.~Christodoulou and E.~Koutsoupias,
``On the Price of Anarchy and Stability of Correlated Equilibria of Linear Congestion Games,''
\emph{European Symposium on Algorithms}, Springer, pp.59-70, 2005.

\bibitem{PoS-2003}
A.S.~Schulz and N.S.~Moses,
``On the Performance of User Equilibria in Traffic Networks,''
\emph{ACM-SIAM Symposium on Discrete Algorithms (SODA)}, pp.86-87, 2003.

\bibitem{PoS-2008}
E.~Anshelevich, \emph{et al.},
``The Price of Stability for Network Design with Fair Cost Allocation,''
\emph{SIAM Journal on Computing},  2008.

\bibitem{PoS-2009}
G.~Christodoulou, \emph{et al.},
``On the Price of Stability for Undirected Network Design,''
\emph{International Workshop on Approximation and Online Algorithms},  Springer, 2009.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{altru-TGC2010}
I.~Caragiannis, \emph{et al.},
``The Impact of Altruism on the Efficiency of Atomic Congestion Games,''
\emph{Int.~Symposium on Trustworthy Global Computing},
Springer, pp.172-188, 2010.

\bibitem{altru-Xu2014}
X.~Chen, X.~Gong, L.~Yang, and J.~Zhang,
``A Social Group Utility Maximization Framework with Applications in Database Assisted Spectrum Access,''
\emph{Proc.~IEEE INFOCOM},  2014.


\bibitem{altru-NAEC2009}
A.P.~Azad, E.~Altman, and R.~Elazouzi,
``From Altruism to Non-Cooperation in Routing Games,''
\emph{Networking and Electronic Commerce Research Conference},  2009.


\bibitem{altru-CDC2010}
G.~Kesidis, Y.~Jin, A.P.~Azad, and E.~Altman,
``Stable Nash Equilibria of Aloha Medium Access Games under Symmetric, Socially Altruistic Behavior,''
\emph{Proc.~IEEE CDC}, pp.1071-1075, 2010.


\bibitem{altru-EC2008}
P.A.~Chen and D.~Kempe,
``Altruism, Selfishness, and Spite in Traffic Routing,''
\emph{ACM Conf.~Electronic Commerce (EC)}, 2008.

\bibitem{altru-INFOCOM2010}
J.~Elias, F.~Martignon, K.~Avrachenkov, and G.~Neglia,
``Socially-Aware Network Design Games,''
\emph{Proc.~IEEE INFOCOM}, 2010.


\bibitem{altru-CSEF2007}
G.~De Marco and J.~Morgan,
``Slightly Altruistic Equilibria in Normal Form Games,''
\emph{Centre for Studies in Economics and Finance (CSEF)}, University of Naples, 2007.

\bibitem{altru-AGT2012}
K.R.~Apt and G.~Schafer, ``Selfishness Level of Strategic Games,''
\emph{Algorithmic Game Theory}, Springer, pp.13-24, 2012.


\bibitem{altru-WINE2011}
P.A.~Chen, B.~de Keijzer, D.~Kempe, and G.~Schafer,
``On the Robust Price of Anarchy of Altruistic Games,''
\emph{Int.~Workshop on Internet and Network Economics}, Springer, pp.383-390, 2011.


\bibitem{altru-ESA2009}
M.~Hoefer and A.~Skopalik,
``Altruism in Atomic Congestion Games,''
\emph{Eur.~Symposium on Algorithms}, Springer,  2009.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{income-tax}
Wikipedia, ``Income Tax,''
\emph{The Free Encyclopedia}, 2016.


\bibitem{common}
J.~Geanakoplos, ``Common Knowledge,''
\emph{Handbook of Game Theory with Economic Applications}, pp.1437-1496, 1994.

\bibitem{max-min}
B.~Radunovic and J.Y.L.~Boudec, ``A Unified Framework for Max-Min and Min-Max Fairness with Applications,''
\emph{IEEE/ACM Transactions on Networking (TON)}, 15(5), pp.1073-1083, 2007.


\bibitem{Nash-bargaining}
J.F.~Nash, ``The Bargaining Problem,''
\emph{Econometrica},  1950.

\bibitem{Shapley-value}
L.S.~Shapley, ``A Value for n-person Games,''
chapter in \emph{Contributions to the Theory of Games}, Princeton Univ Press,  2016.

\bibitem{hitl}
G.~Schirner, D.~Erdogmus, \emph{et al.},
``The Future of Human-In-The-Loop Cyber-Physical Systems,''
\emph{Computer}, 2013.


\bibitem{im-theory}
E.~Maskin and T.~Sjostrom, ``Implementation Theory,''
\emph{Handbook of social Choice and Welfare}, pp.237-288, 2002.

\bibitem{mech-design}
L.~Hurwicz and S.~Reiter, \emph{Designing Economic Mechanisms}, Cambridge University Press, 2006.






%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{xxx-1}
N.D.~Lane, E.~Miluzzo, \emph{et al.}, ``A Survey of Mobile
Phone Sensing,''
 \emph{IEEE Communications Magazine}, 48(9), 2010.

\bibitem{xxx-2}
H.~Ma, D.~Zhao, and P.~Yuan, ``Opportunities in Mobile Crowd Sensing,'' \emph{IEEE Communications Magazine}, 52(8), 29-35, 2014.

\bibitem{xxx-3}
Z.~Feng, \emph{et al}, ``TRAC: Truthful Auction for Location-Aware Collaborative Sensing in Mobile Crowdsourcing,''
\emph{Proc. IEEE INFOCOM},  2014.

\bibitem{xxx-4}
%L.~Gao, F.~Hou, and J.~Huang, ``Providing Long-Term Participation Incentive in Participatory Sensing,''
%\emph{Proc. IEEE INFOCOM},  2015.
M. H. Cheung, \emph{et al.}, ``Distributed time-sensitive task selection in mobile crowdsensing,'' \emph{Proc. ACM MobiHoc}, 2015.


\bibitem{xxx-5}
X. Sheng, J. Tang, and W. Zhang, ``Energy-efficient
collaborative sensing with mobile phones,''
\emph{Proc. of IEEE INFOCOM}, 2012.

\bibitem{xxx-6}
Q. Zhao, \emph{et al.}, ``Fair energy-efficient sensing task allocation in
participatory sensing with smartphones,
\emph{Proc. of IEEE INFOCOM}, 2014.


\bibitem{mcs-app1}
WeatherLah, http://www.weatherlah.com/.

\bibitem{mcs-app2}
Intel Urban Atmosphere, http://www.urban-atmospheres.net/.

\bibitem{mcs-app3}
OpenSignal, http://opensignal.com/.

\bibitem{mcs-app4}
Waze: Free GPS Navigation with Turn by Turn, https://www.waze.com/.


\bibitem{xxx-potential}
D.~Monderer and L.S.~Shapley, ``Potential Games,'' \emph{Games and economic behavior}, 14(1), 124-143, 1996


\bibitem{yyy-1}
G.~Iosifidis, \emph{et al.}, ``Enabling Crowd-Sourced Mobile Internet Access,'' \emph{Proc. IEEE INFOCOM}, 2014.

%\bibitem{yyy-2}
%OpenGarden Inc., url: http://opengarden.com/


\bibitem{report}
Online Technical Report, available at Dropbox,
url:
\\
www.dropbox.com/s/uordjn48q53ln32/AppTAX.pdf?dl=0


\end{thebibliography}


